Escaping from Zero Gradient: Revisiting Action-Constrained Reinforcement Learning via Frank-Wolfe Policy Optimization

Action-constrained reinforcement learning (RL) is a widely-used approach in various real-world applications, such as scheduling in networked systems with resource constraints and control of a robot with kinematic constraints. While the existing projection-based approaches ensure zero constraint violation, they could suffer from the zero-gradient problem due to the tight coupling of the policy gradient and the projection, which results in sample-inefficient training and slow convergence. To tackle this issue, we propose a learning algorithm that decouples the action constraints from the policy parameter update by leveraging state-wise Frank-Wolfe and a regression-based policy update scheme. Moreover, we show that the proposed algorithm enjoys convergence and policy improvement properties in the tabular case as well as generalizes the popular DDPG algorithm for action-constrained RL in the general case. Through experiments, we demonstrate that the proposed algorithm significantly outperforms the benchmark methods on a variety of control tasks.

==> 04-analysis.tex <==
\section{Convergence Results}

==> 06-num.tex <==
\section{QoE-Based Network Utility Maximization}
\label{section:NUM}

%\subsection{Budget Constraint on Total Playback Latency}


%\subsection{Constraint on Frame Dropping Rate}


%\subsection{Fixed $D_n(t)$ to $d_n$ ratios}

==> 07-exp-backup.tex <==
\section{Experimental Results}
\label{section:exp}
In this section, we evaluate the proposed learning algorithm via experiments on control tasks in various domains, including communication networks, bike sharing systems, and continuous control tasks on the MuJoCo suite.

We compare the proposed algorithms against the following four popular baseline methods:

\begin{itemize}[leftmargin=*]
    \item \textbf{DDPG}: The vanilla version of DDPG proposed in \citep{lillicrap2016continuous}.
    \vspace{-0mm}-
    \item \textbf{DDPG+Projection}: The training procedure is identical to DDPG except that the action is post-processed by $L_2$-projection before being applied to the environment.
    \vspace{-0mm}
    \item \textbf{DDPG+RewardShaping}: Built on DDPG+Projection, this algorithm adds the $L_2$-norm between the primitive action and its projection as a penalty to the intrinsic reward.
    \vspace{-4mm}
    \item \textbf{DDPG+OptLayer}: This design uses a differentiable projection layer, namely the OptLayer, that supports end-to-end training via gradient descent \citep{pham2018optlayer}. To implement the OptLayer, we leverage the open-source packages cvxpylayer \citep{agrawal2019differentiable} as well as the OptNet proposed by \citep{amos2017optnet}. 
\end{itemize}
%DDPG , DDPG with OptLayer\cite{pham2018optlayer}, which an additional projection layer, and DDPG with reward shaping, add an additional projection loss penalty($P$) to reward, 
%\begin{equation}
%P = D\sum_{i=0}^n(a_i-a_i^*)^2 , a_i^*\in \cC(s)
%\end{equation}
%where $a_i^*$ is the closet  projection point to $a_i$ and also satisfy the constraint, $D$ is a scalar differ in each environment, so the reward $r$ become $r-P$; the last method is DDPG+Projection, only project the action into $\cC(s)$ without gradient information for the projection step.
%In NFWPO, DDPG+Reward Shaping, and DDPG+Projection, a projection step after the output of the actor network is involved. Here we leverage Gurobi Solver \cite{gurobi} for this projection process. In DDPG+OptLayer, we add an additional differentiable OptLayer at the output of the policy network, which leverages open-source packages cvxpylayer \cite{agrawal2019differentiable} and qpth solver proposed by \cite{amos2017optnet}. 

We use the architecture of DDPG \citep{lillicrap2016continuous} as the base for all the algorithms. For both the actor and critic networks, we use two hidden layers with 400 and 300 hidden units with ReLU as the activation. For the activation function of the actor output, in order to better accommodate the various action ranges of different environments, we choose tanh for the MuJoCo continuous control tasks and ReLU for the other tasks, respectively. %For the critic, we do not include actions until the second hidden layer. 
%The parameters of the target network are softly updated with an update rate $\tau = 10^{-3}$. 
%The discount factor is $\gamma = 0.99$.
%The parameters of the main actor and critic network are updated using the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$ for the actor and $10^{-3}$ for the critic. 
For the projection step (without the need of backpropagation) required by DDPG+Projection, DDPG+RewardShaping, and FWPO/NFWPO, we implement this functionality on the Gurobi optimization solver \citep{gurobi}.
%A mini-batch is randomly sampled from the experience replay buffer and is trained after each time step, with mini-batch size of 16 for NFWPO and DDPG+OptLayer, and 64 for DDPG+Reward Shaping and DDPG+Projection. The actor network is lazy updated every 50 steps in DDPG+OptLayer, while the others are still updated every steps. 
%For the additional projection layer, we leverage the open-source package cvxpylayers \cite{agrawal2019differentiable}. The complete comparison of hyper-parameter choices is provided in Table \ref{tab:hyperParam}.
For each task, each algorithm is trained under the common set of 5 random seeds. Each evaluation consists of 10 episodes, and we report the average performance along with the standard deviation.

\textbf{Bike Sharing Systems.}
We use the open-source simulator gym-BSS \footnote{https://github.com/bhatiaabhinav/gym-BSS}, which was proposed by \citep{ghosh2017incentivizing} and is built on the OpenAI Gym interface. 
%In Bike Sharing, we use tabular for action decision.
%In the Bike Sharing, it simulate the bike renting system, 
In a bike sharing environment, there are $m$ bikes and $n$ stations, each of which has a pre-determined bike storage capacity $C$. 
At each time step, for each pair of stations $i,j$, there are random demands of 5 to 25 bikes from station $i$ to $j$.
An action is to allocate the $m$ bikes to $n$ station in order to maximize the total reward. 
This indicates that an action is $n$-dimensional.
The reward consists of three terms: (i) Moving cost: the cost of moving one or multiple bikes from one station to another; (ii) Lost-demand cost: the cost of unserved demand due to bike outage. (iii) Overflow cost: the cost incurred by the event that the number of bikes in one station exceeds its capacity (due to the random demand). 
%Next we discuss the tabular setting and the constraint detail.

As the bike sharing environment has a finite state space, we first use it to evaluate FWPO with tabular policy parameterization.
We choose a medium-sized system with $m=90$, $n=3$, and $C=35$, which allows us to analytically find the optimal policy for this environment.
There are two types of action constraints: (i) Global constraint: the sum of the entries of an action shall be equal to $90$; (ii) Local constraints: each entry of the action shall be between $0$ and $35$.
%\begin{itemize}[leftmargin=*]
%    \item Global constraint: the sum of the entries of an action shall be equal to $90$.
%    \vspace{-2mm}
%    \item Local constraints: each entry of the action shall be between $0$ and $35$.
%\end{itemize}
%Bike Sharing Tabular case : In tabular case, we decrease the zone to three, therefore, the action has only 3-dim to decide how many bikes need in the particular zone correspond to the state, so we can update our policy base on the action table, then update the action table by each algorithm. The constraint of tabular case is
%Local constraint : $\forall_i0<=a_i<=35$
%\vspace{-2mm}
We exclude the neural-based approach DDPG+OptLayer from the comparison for this tabular environment.
%is not included for comparison because there is no policy network, only policy table. 
%The reason why we use tabular case is because we can calculate the optimal solution by Markov Decision Process. And by our calculation, the optimal policy of 3-zone Bike-sharing is to choose action equal to state, which equal to not move the bike, because the moving cost we set is one for each bike, the cost of moving bike is very high, also the reward can tune to whenever we want and still can get the other optimal solution, and the explore technique is changing from Gaussian noise to epsilon greedy with 0.1 probability that random sample the action, because of the variety of action space. 
%The policy table is initialized by $(20,35,35)$ bikes for the three zones in every state. 

Figure \ref{fig:Bike all}(a) shows the average return of the three algorithms. 
FWPO indeed performs the best, while DDPG-Projection and DDPG+RewardShaping both suffer from slow learning.
This also can be reflected by Figure \ref{fig:Bike all}(b), which shows the distance between the learned policies and the optimal policy.
We observe that FWPO converges to a near-optimal policy much faster than the baselines.
This above phenomenon is mainly due to the inaccurate policy gradient of DDPG:
The critic networks of the two baselines fail to provide since the policy gradient (\textit{cf.} \ref{eq:sample-based DPG}) of is evaluated at those actions outside the feasible sets while the samples in the replay buffer .
As FWPO always stays in the feasible action sets, it naturally avoids the issue of inaccurate gradients.

%evaluation reward and norm difference between optimal policy are shown in .


\textbf{Utility Maximization of Communication Networks.}
%For utility maximization of communication networks, w
We use the open-source network simulator from PCC-RL \footnote{PCC-RL: https://github.com/PCCproject/PCC-RL} \citep{jay2019internet} built on the OpenAI Gym interface and implement the additional functionalities for our experiments. 
%Network-sim provides a simulation gym to show how networks work. 
For the network topology, we consider the classic T3 NSFNET Backbone \footnote{T3 NSFNET: https://en.wikipedia.org/wiki/National\_Scien-ce\_Foundation\_Network} and set the bandwidth of each link to be 50 packets per second throughout the experiments.
%For our implementation of network, 
We create three network flows, each of which has three candidate paths from its source to the destination. 
The action is to determine the rate allocation of each flow along each candidate path, and therefore the action is 9-dimensional. 
%allocate the flow the packets to distinct paths and their corresponding flows
%Every term of action represents the amount of packets transmitted on the corresponding path. 
The reward consists of three terms: (i) Throughput: the number of received packets per second; (ii) Drop rate: the number of dropped packets per second; (iii) Latency: the average latency of the packets in the last second. For each flow $i$, its immediate reward is $\log({\frac{\text{throughput}_{\bf i} }{\text{drop}_{\bf i}^{0.5} \times \text{latency}_{\bf i}^{1.5}} })$, which corresponds to the widely-used proportional fairness criteria \citep{kelly1997charging}.
%it has an utility function $U(i)$
% \begin{align}
%  &U_i = \log\Big({\frac{\text{throughput}_{\bf i} }{\text{drop}_{\bf i}^{0.5} \times \text{latency}_{\bf i}^{1.5}} } \Big)
% \end{align}
%, and we want to maximize the reward 
% \begin{equation}
% \textbf{reward} =  \sum_{i=1}^{3} U(i) \\
% \end{equation}
%where \textbf{throughput} , \textbf{drop} and \textbf{latency} are measured in packets each flow. 
One salient feature of a communication network is that when the total packet arrival rate of a link approaches its bandwidth, the latency will grow rapidly, and accordingly most of the packets would be dropped. 
Therefore, in this environment, the action constraints correspond to the link capacity constraints, i.e., the total assigned packet arrival rate of each link should be upper bounded by 50. 
%Therefore, before we perform different actions to distribute packets, we should make sure that the total amount of packet allocation for each link cannot exceed its bandwidth. For every link $i$, we have a utility $Ut(i)$
%  \begin{align}
% &Ut(i) = \sum {a_j} 
% \end{align}
%$a_j$ represents the path through link $i$. We impose the constraint base on the action. 
%  \begin{align}
% &Ut(i) <= 50
% \end{align}

Figure \ref{fig:Network all}(a) shows the training curve of NFWPO and the baseline algorithms.
We can observe that NFWPO converges fast (in about $10^5$ steps) and achieves much larger average return than the other baselines.
Interestingly, Figure \ref{fig:Network all}(b) indicates that the primitive actions of NFWPO can already largely avoid constraint violation, and therefore NFWPO requires the help of the projection step only for a small portion of training steps.
By contrast, the other two baseline methods make only little progress in acquiring the rewards or adapting to the constraints, even for DDPG+RewardShaping with the guidance of a penalty based on the constraint violation.
 
\begin{figure*}[!tb]
\centering
$\begin{array}{c c}
    \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }}   \\ 
    \hspace{-1mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/NSFnetV2_reward.eps}}  \label{fig:Network_reward} & 
    \hspace{-3mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/NSFnetV2_con.eps}} 
    \label{fig:Network_constraint_violate} \\
    \mbox{\small (a)} & \hspace{-2mm} \mbox{\small(b)}%\mbox{\small (b)} & \hspace{-2mm} 
\end{array}$
\caption{Utility maximization in NSFNET: (a) Average return at each evaluation over 5 random seeds; (b) {Cumulative number of constraint violations of the primitive actions during training.}}
\label{fig:Network all}
\end{figure*}


\begin{figure*}[!tb]
\centering
$\begin{array}{c c}
    \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }}   \\ 
    \hspace{-1mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Bike_tabular_reward.eps}}  \label{fig:Bike_sharing_reward} & 
    \hspace{-3mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Bike_tabular_norm.eps}}
    \label{fig:Bike_sharing_norm} \\
    \mbox{\small(a)} & \hspace{-2mm} \mbox{\small(b)}%\mbox{\small (b)} & \hspace{-2mm} 
\end{array}$
\caption{Bike sharing systems: (a) Average return at each evaluation over 5 random seeds; (b) The $L_2$-norm between the learned policy and the optimal policy at each training step.}
\label{fig:Bike all}
\end{figure*}

\begin{figure*}[!tb]
\centering
$\begin{array}{c c c}
    \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }} \\ 
    \hspace{-0mm} \scalebox{0.34}{\includegraphics[width=\textwidth]{./figures/Bike_Grad_3.eps}}  \label{fig:Bernoulli_ID=2_Regret_T=1e5} & 
    \hspace{-5mm} \scalebox{0.34}{\includegraphics[width=\textwidth]{./figures/Bike_net_reward.eps}} \label{fig:Gaussian_ID=16_Regret_T=1e5} & \hspace{-5mm}
    \scalebox{0.34}{\includegraphics[width=\textwidth]{./figures/Bike_net_cons.eps}} \label{fig:Exp_ID=21_Regret_T=1e5}\\ [0.0cm]
    \mbox{\hspace{-0mm}\small (a)} & \hspace{-2mm} \mbox{\small (b)} & \hspace{-2mm} \mbox{\small (c)} \\[-0.2cm]
\end{array}$
\caption{Bike sharing systems:(a)Zero Gradient in OptLayer, the $log-L_2$ norm gradient before OptLayer is close to zero; (b) Average return at each evaluation over 5 random seeds; (c) Cumulative number of constraint violations of the primitive actions during training.}
\label{fig:regret all}
\end{figure*}


\textbf{MuJoCo Continuous Control Tasks.}
For robotic systems with kinematic constraint, we use MuJoCo continuous control tasks to evaluate the proposed algorithm for both linear, non-linear and state-dependent action constraints \citep{6386109}. We consider two control tasks, namely Reacher-v2 and Halfcheetah-v2. %( 2-dim action space and 11-dim state space, and Halfcheetah-v2:8-dim action space and 17-dim state space.)
In Reacher-v2, the state space is 11-dimensional, and the action space is $2$-dimensional (denoted by $u_{1},u_{2}$). 
Each entry of an action corresponds to the torque of a joint of a 2-dof robot.
We impose the action constraints as $\lvert u_{1}+u_{2}\rvert\leq 0.1$ and $ {u_{1}}^2+{u_{2}}^2\leq 0.02$.
%base on the action, which make the action behave safety to catch the goal, and , the reward is base on the distance of the goal and the action control cost. The constraints of Reacher-v2 are show below.
%Reacher-v2 :
On the other hand, the action space of Halfcheetah-v2 is $6$-dimensional (denoted by $v_{1},\cdots,v_{6}$).
We consider two instances of action constraints separately: (i) Quadratic constraints (Halfcheetah-Quad): $v_1^2+v_2^2+v_3^2\leq 1$, $v_4^2+v_5^2+v_6^2\leq 1$; (ii) State-dependent constraint (Halfcheetah-State): $\sum_{i=1}^{6} |v_i w_i|\leq 20$, where $w_i$ denotes the angular velocity of the $i$-th joint. This constraint is meant to capture the output power constraint.
\vspace{-2mm}

%\begin{itemize}[leftmargin=*]
%    \item Quadratic constraints: $v_1^2+v_2^2+v_3^2\leq 1$, $v_4^2+v_5^2+v_6^2\leq 1$.
%    \vspace{-2mm}
%    \item State-dependent constraint: $\sum_{i=1}^{6} |v_i w_i|\leq 20$, where $w_i$ denotes the angular velocity of the $i$-th joint. This constraint is meant to capture the output power constraint of the robot.
%\end{itemize}


%is a planar biped robot with each side 3 joint(thing, shin, foot) to control the robot to run as fast as it can to get the forward reward, thus the action is 6-dim, and the action also need to balance the cost of control reward at the same time, the state space is 17-dimension. In half-cheetah, we experiments on two setting, the goal of the first one is to make sure the action behave safety to control the robot, and the second one is based on the power which makes the robot forward less effort. Below are the two experiments constraint.

%Halfcheetah-Cons-1 : 
%$a_1^2+a_2^2+a_3^2<=1$ and $a_4^2+a_5^2+a_6^2<=1$

%Halfcheetah-Power (state-related constraint): 
%$\sum_{i=1}^{6} |a_i*w_i|$ where $w_i$ is correspond to the angular velocity of joint $i$.

The results are shown in Figure \ref{fig:Reacher all} and Figure \ref{fig:Halfcheetah all}.
Similar to the other environments, we still observe that FWPO achieves better sample efficiency than the other baselines and has much fewer constraint violations in the primitive actions.

%contain the average return, and the constraint violate term for each step during training, the less violate, the more accurate the network aware of the constraint and can find the much better solution in each.
Finally, we summarize the average return over the final 10 evaluations in Table \ref{tab:expResult}. 
%The learning curves and the constraint violation during training are presented in Figure \ref{fig:Halfcheetah all}. 
%NFWPO outperforms all other algorithms in both final performance and learning speed across all tasks. Moreover, NFWPO has the least constraint violation compared to the baselines.


\begin{figure*}[!tb]
\centering
$\begin{array}{c c}
    \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }}   \\ 
    \hspace{-1mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Reacher_reward_eps.eps}}  \label{fig:Reacher_reward} & 
    \hspace{-3mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Reacher_cons.eps}}
    \label{fig:Reacher_constraint_violate} \\
    \mbox{\small (a)} & \hspace{-2mm} \mbox{\small(b)}%\mbox{\small (b)} & \hspace{-2mm} 
\end{array}$
\caption{Reacher-v2: (a) Average return at each evaluation over 5 random seeds; (b) {Cumulative number of constraint violations of the primitive actions during training.}}
\label{fig:Reacher all}
\end{figure*}
\vspace{-2mm}

\begin{figure*}[!tb]
\centering
$\begin{array}{c c c c}
    \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }}  \\ 
    \hspace{5mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Halfcheetah_1_reward.eps}}  \label{fig:Halfcheetah-1-reward} & 
    \hspace{0mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Half_state_relate_reward.eps}}
    \label{fig:Halfcheetah-SR-reward} \\
    \mbox{\hspace{6mm}\small (a)} & \hspace{0mm} \mbox{\small(b)} \\
     \hspace{5mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Halfcheetah_1_cons.eps}}  \label{fig:Halfcheetah-1-violate} & 
    \hspace{0mm} \scalebox{0.35}{\includegraphics[width=\textwidth]{./figures/Half_state_relate_cons.eps}}
    \label{fig:Halfcheetah-SR-violate} \\
    \mbox{\hspace{6mm}\small (c)} & \hspace{0mm} \mbox{\small(d)}
\end{array}$
\caption{Halfcheetah-v2: (a)-(b) Average returns under the quadratic constraints and the state-dependent constraint, respectively; (c)-(d) Cumulative number of constraint violations of the primitive actions during training under the quadratic constraints and the state-dependent constraint, respectively.}
\label{fig:Halfcheetah all}
\end{figure*}


\begin{comment}
\begin{figure*}[!tb]
\centering
$\begin{array}{c c c c c c}
    \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }} & \multicolumn{1}{l}{\mbox{\bf }} \\ 
    \hspace{-1mm} \scalebox{0.33}{\includegraphics[width=\textwidth]{2021_ICML_FWPO/figures/Half_cheetah_Cons1_ Average Reward_true.pdf}}  \label{fig:Bernoulli_ID=2_Regret_T=1e5} & 
    \hspace{-3mm} \scalebox{0.33}{\includegraphics[width=\textwidth]{2021_ICML_FWPO/figures/Reacher Average Reward_true.pdf}} \label{fig:Gaussian_ID=16_Regret_T=1e5} & \hspace{-3mm}
    \scalebox{0.33}{\includegraphics[width=\textwidth]{2021_ICML_FWPO/figures/Half_4.pdf}} \label{fig:Exp_ID=21_Regret_T=1e5}\\ [0.0cm]
    \mbox{\small (a)} & \hspace{-2mm} \mbox{\small (b)} & \hspace{-2mm} \mbox{\small (c)}\\
    \hspace{-1mm} \scalebox{0.33}{\includegraphics[width=\textwidth]{2021_ICML_FWPO/figures/Half_cons1_violate.pdf}}  \label{fig:Bernoulli_ID=2_Regret_T=1e5} & 
    \hspace{-3mm} \scalebox{0.33}{\includegraphics[width=\textwidth]{2021_ICML_FWPO/figures/Reacher Average Reward_true.pdf}} \label{fig:Gaussian_ID=16_Regret_T=1e5} & \hspace{-3mm}
    \scalebox{0.33}{\includegraphics[width=\textwidth]{2021_ICML_FWPO/figures/THIS.pdf}} \label{fig:Exp_ID=21_Regret_T=1e5}\\ [0.0cm]
    \mbox{\small (d)} & \hspace{-2mm} \mbox{\small (e)} & \hspace{-2mm} \mbox{\small (f)}
    \\[-0.2cm]
\end{array}$
\caption{Halfcheetah-v2: (a)(b)(c) Average Return of each constraint(Halfcheetah-Cons-2.25,Halfcheetah-Cons-1,Halfcheetah-Power) (d)(e)(f)Cumulative constraint violation during training before Gaussian noise of each constraint(Halfcheetah-Cons-2.25,Halfcheetah-Cons-1,Halfcheetah-Power) }
\label{fig:Halfcheetah all}
\end{figure*}
\end{comment}

\begin{table*}[!tb]
    \centering
    % \setlength{\tabcolsep}{} %% default is 6pt
    \caption{Average return over the last 10 evaluations over 10 trials.}
    \label{tab:expResult}
    \begin{tabular}{l c c c c c c}
         \hline Methods & Reacher & Halfcheetah-Quad & Halfcheetah-State & NSFNET & BSS-3 & BSS-5 \\
         \hline
         NFWPO & \textbf{-7.18814} & \textbf{4948.45} & \textbf{6513.26} & \textbf{11988.67} & \textbf{-1673.04} & \textbf{-15248.5} \\
         DDPG+Projection & -12.1004 & 1325.21 & 2746.72 & 1515.74 & -2254.52 & -16124.9 \\
         DDPG+Reward Shaping & -10.1051 & 2133.05 & 3065.37 & 4750.66 & -2308 & -16124.9 \\
         DDPG+OptLayer & -8.0951 & 3820.25 & 539.461 & 2440.99 & - & -16693.4  \\
         \hline
    \end{tabular}
\end{table*}
